Risks and Opportunities of Open-Source Generative AI

Applications of Generative AI (Gen AI) are expected to revolutionize a number of different areas, ranging from science & medicine to education. The potential for these seismic changes has triggered a lively debate about the potential risks of the technology, and resulted in calls for tighter regulation, in particular from some of the major tech companies who are leading in AI development. This regulation is likely to put at risk the budding field of open-source generative AI. Using a three-stage framework for Gen AI development (near, mid and long-term), we analyze the risks and opportunities of open-source generative AI models with similar capabilities to the ones currently available (near to mid-term) and with greater capabilities (long-term). We argue that, overall, the benefits of open-source Gen AI outweigh its risks. As such, we encourage the open sourcing of models, training and evaluation data, and provide a set of recommendations and best practices for managing risks associated with open-source generative AI.

==> sections/3_regulatory/3_regulatory.tex <==
\newpage
\section{Regulatory Landscape, Governance and Geopolitics}

==> sections/5_medium_term/5_medium_term.tex <==
\section{Medium-term Impact of Open Source Models}

==> sections/8_recommendations/8A_debunking.tex <==
\section{Addressing Common Concerns when Open Sourcing Generative AI}
\label{sec:debunking}


%In the academic community, there is a prevailing consensus that the open-sourcing of General Artificial Intelligence (Gen AI) would facilitate the comprehensive and widespread realization of its benefits. 
%However, the contentious aspect lies in the apprehension that open-sourcing Gen AI could potentially escalate both the frequency and severity of its malicious applications \citep{seger2023open}. 
%Notwithstanding the existence of a faction opposed to the advancement of more sophisticated models, regardless of their open or closed-source nature, the predominant view does not advocate for a complete cessation of Gen AI development. 
%The crux of the debate centers on the question of whether the incremental risks associated with open-sourcing Gen AI models, as opposed to maintaining them as closed-source, are justifiable. 
%We believe that the perceived amplification of these risks is exaggerated and sometimes motivated by economic reasons and aim to address several of the predominant concerns.
Despite the many benefits of open source, concerns surrounding the increased potential for malicious use, and uncertainty about its societal impact, have prompted calls for keeping generative AI closed source \citep{seger2023open}. There are real risks associated with open source models. However, we believe these are sometimes exaggerated, possibly motivated by the economic interests of market leaders. Most concerns about open sourcing near to mid-term AI models are also pertinent to closed source models.
%Instead, hard restrictions on open sourcing might not yield large improvements in overall safety, and could even hinder advancements in open safety technologies and auditing procedures. 
In this section, we aim to address some of the primary concerns typically raised in favor of closed source Gen AI models. 
%To safely and responsibly open source Gen AI models, we outline important priorities moving forward, starting with technical recommendations before moving to broader responsibility and socio-technical considerations.
%Most apprehensions associated with open sourcing near to mid-term Gen AI are also pertinent to closed source models. 


\textbf{CLAIM \#1: Closed Models Have Inherently Stronger Safeguards than Open Source Models.}
Several studies demonstrate that closed models typically demonstrate fewer safety and security risks, compared to open source \cite{rottger2023xstest, chen2024chatgpts, sun2024trustllm}. 
However, closed models still demonstrate weaknesses and are particularly vulnerable to jailbreaking techniques \citep{zou2023universal,chao2023jailbreaking}.
Closed model safeguards are easily bypassed through simple manipulations like fine-tuning via accessible services \citep{qi2023fine}, prompting the model to repeat a word \citep{nasr2023scalable}, applying a cypher \cite{yuan2023gpt4}, or instructing the model in another language \citep{deng2023multilingual,yong2023low}.
Completely preventing models from exhibiting undesirable behaviors might not even be possible \citep{wolf2023fundamental,petrov2024prompting}.
Therefore, it is not clear that closed models are definitively ``safer'' than open source models. We also anticipate that gaps will narrow over time as jailbreaking attacks become stronger and open safeguarding methods continue to improve. 
% The robustness of closed source models' safeguards is debatable. 
% The field of creating jailbreaks for these models has rapidly advanced and achieved notable successes \citep{zou2023universal,chao2023jailbreaking}. 
% Additionally, a malignant objective can be deconstructed into benign subtasks processed by a closed model, and subsequently reassembled using a less sophisticated open-source model.
% The distinction between benign and malicious usage, akin to, e.g., the use of virology knowledge, often hinges on contextual application, a nuance typically absent in closed models. 
% Thus, they cannot inherently discern the intent of use.
% \textbf{Closed Models Might Pose Some Risks With, e.g., Sophisticated Jailbreaks, but Open-Source Models Have Higher Ease of Access }
% Regarding intentional harms, a determined malicious actor will likely find a way to exploit a closed model. 
% Currently, there are private networks sharing jailbreaks and exploits confidentially as to not have them patched by the model providers \citep{jailbreakMarket}. 
% As far as unintentional harms are concerned (\Cref{sec:safety}), open-source models parallel the role of Linux in the technology ecosystem -- essential in the background but not predominantly used by the general public, unlike commercial platforms like MacOS and Windows.

\textbf{CLAIM \#2: Access to Closed Models Can Always be Restricted.}
Closed models are often considered more secure because access can be restricted or removed should issues be identified. However, closed models can be compromised via hacking, leaks \citep{llamaLeak}, reverse engineering \citep{appleHack} or duplication \citep{Oliynyk2023stealing}. 
This perspective also assumes that models are only offered through an API. But some closed models are delivered on premise/device, particularly for sensitive deployments (e.g., government applications). In such cases, access may not be retractable.
Finally, closed models can be leaked, e.g., Mistral's 70B parameter was leaked by one of their early customers \citep{franzen2024}. 
Given these factors, developers of closed models do not always have the ability to unilaterally revoke access.
% It does not hold for an alternative approach where the model weights are sold, resembling proprietary source-available software. 
% This latter approach is particularly relevant for on-device applications or sensitive deployments, such as in government institutions.
% In such scenarios, the developer loses the ability to unilaterally restrict access if customers operate their own instances of the model. 

\textbf{CLAIM \#3: Closed Source Developers Can be Regulated to be Safer.}
Regulatory pressure is primarily aimed at large companies building closed source models. For instance, the  \href{https://www.whitehouse.gov/briefing-room/statements-releases/2023/10/30/fact-sheet-president-biden-issues-executive-order-on-safe-secure-and-trustworthy-artificial-intelligence/}{White House Executive Order} required 15 ``leading companies'' to ``drive safe, secure, and trustworthy development of AI.''
Regulatory pressure is a lever for society to create incentives for safe model development. However, regulation is not a panacea and several closed source models have been, and could be, released that are uncensored, poorly safeguarded \citep{elevenScam} or deliberately misaligned \citep{wormGPT,Grok1,Grok2}. 
It is also not clear that regulating closed source models is an effective way of stopping malicious actors \citep{yakuza,NigerianScammers}, who do not comply with regulation and are capable of creating and distributing their own closed source models via illicit sales channels \citep{AiCybercriminal}. 
Instead, regulation might create higher costs for legitimate users who are restricted in what models they can access, develop and share \citep{wu2023llmdet}.
% Additionally, the absence of open source counterparts to these powerful models may not significantly impede malicious actors
% , as the latter can still access models crafted by unauthorized or illicit organizations for malicious purposes.
% requires companies like 
% This provides a mechanism for societal 
% through initiatives such as  and industry-wide collaborations. 
% The prevailing assumption that closed-source developers inherently bolster the safety and security of their systems, often under regulatory pressure, warrants reconsideration. In practice, the development and deployment of uncensored,
% The lack of potent open-source models potentially hinders legitimate users more severely than malevolent ones


\textbf{CLAIM \#4: All Safety and Security Problems Must be Addressed By the Model Provider.}
% Assessing the risks created by AI models is an open area of research \cite{rottger2023xstest, vidgen2023simplesafetytests, weidinger2023}. 
It is becoming increasingly clear that, because of the numerous potential applications of generative models, all safety risks cannot be simply identified (and addressed) by the model provider. 
First, most model-related risks depend on access to real-world resources. 
However, legal, financial, and physical constraints significantly hinder activities like acquiring chemicals, equipment and tacit know-how, thus limiting open source's potential for misuse for developing chemical, bio and conventional weapons. 
It is crucial to recognize that effective mitigation of these risks often lies beyond the digital realm. 
% Second, models may not have a causal impact on actors if they either (a) have other means of inflicting harm -- such as searching on the web for malicious information -- or (b) pay little attention to the responses of the model.
Internet Service Providers (ISPs), cloud service providers, social media platforms, along with law enforcement and intelligence agencies, have developed robust measures to mitigate these threats.
This highlights a critical aspect: the potential harm of Gen AI is not determined by access to information but by the capacity to act upon it, which is the same for open and close source models.
% Consequently, it is imperative to acknowledge that substantial mechanisms to prevent misuse exist outside the Gen AI system, rooted in the physical and regulatory landscapes.
% Third, in practice, other stakeholders help protect people from risk through established safeguarding practices, such as Internet Service Providers, cloud services, social media, and law enforcement. 
Given these factors, safety and security issues cannot be seen as solely the responsibility of the model provider and substantial mechanisms to prevent misuse exist outside the Gen AI system, rooted in the physical and regulatory landscapes. 

% This underscores that the potential for Gen AI harm depends not just on information access but also on the ability to act, highlighting the importance of external, non-digital safeguards in mitigating misuse.
%Moreover, digital risks, including scams and disinformation, are being effectively addressed by 
% It is often argued that open source models have more risks than closed source ones. However, in discussing generative AI risks, it's vital to note that risk mitigation extends beyond the digital, encompassing legal, financial, physical, and regulatory challenges. 
% In the discourse on the risks associated with generative AI models, it is crucial to recognize that effective mitigation of these risks often lies beyond the digital realm. 
% The majority of AI-related risk scenarios hinge on the ability to navigate a multitude of real-world hurdles, including legal, financial, and physical constraints, as well as stringent oversight and regulatory frameworks. 
% For instance, scenarios that involve tangible actions—such as acquiring chemical components, laboratory equipment, or weaponry—are significantly impeded by existing real-world barriers. 
% These barriers limit the extent to which open-source Gen AI models can facilitate such endeavors.
% Risks situated within the digital domain, such as scams and the spread of disinformation, are already being effectively countered by various entities. 
% Internet Service Providers (ISPs), cloud service providers, social media platforms, along with law enforcement and intelligence agencies, have developed robust measures to mitigate these threats. This highlights a critical aspect: the potential harm of Gen AI is not solely determined by access to information but also by the capability to act upon it. 
% Consequently, it is imperative to acknowledge that substantial mechanisms to prevent misuse exist outside the Gen AI system, rooted in the physical and regulatory landscapes.


%More importantly, it would result in profound setbacks in harnessing the full potential of Generative AI, particularly in terms of its benefits for underrepresented and oppressed communities, as well as for regions in the Global South.




% \{\color{red} For the debunking section: currently available commercial models are not being released purely for safety reasons -- economic reasons are involved too. Accumulation of power is also something we might want to mention.}

% PR Notes
%There are both benefits and risks to open-sourcing generative AI models developed in the near- to mid-term.
%However, there are clear steps to be taken during and after release to mitigate the risks we highlighted throughout this paper.
%We believe that such a \textit{responsible} approach to open-sourcing AI can ensure that the many benefits clearly outweigh the potential downsides.
%By "responsible", we mean that during and after release, steps are taken to mitigate the risks we highlighted throughout this paper.

